Deep Generation of Coq Lemma Names Using Elaborated Terms

Coding conventions for naming, spacing, and other essentially stylistic properties are necessary for developers to effectively understand, review, and modify source code in large software projects. Consistent conventions in verification projects based on proof assistants, such as Coq, increase in importance as projects grow in size and scope. While conventions can be documented and enforced manually at high cost, emerging approaches automatically learn and suggest idiomatic names in Java-like languages by applying statistical language models on large code corpora. However, due to its powerful language extension facilities and fusion of type checking and computation, Coq is a challenging target for automated learning techniques. We present novel generation models for learning and suggesting lemma names for Coq projects. Our models, based on multi-input neural networks, are the first to leverage syntactic and semantic information from Coq's lexer (tokens in lemma statements), parser (syntax trees), and kernel (elaborated terms) for naming; the key insight is that learning from elaborated terms can substantially boost model performance. We implemented our models in a toolchain, dubbed Roosterize, and applied it on a large corpus of code derived from the Mathematical Components family of projects, known for its stringent coding conventions. Our results show that Roosterize substantially outperforms baselines for suggesting lemma names, highlighting the importance of using multi-input models and elaborated terms.

==> figures/architecture.tex <==
\begin{figure}[t]
  \centering
  {\footnotesize
  \begin{tikzpicture}
    \tikzset{node distance=3.5cm, every state/.style={thick},
      initial text={},
      double distance=2pt,
      every edge/.style={
        draw,
        color=black,
        >=stealth',
        auto,
        thick}
    }
    \tikzset{every state/.append style={rectangle,
        inner sep=4pt,
        minimum width = 1cm,
        text=black,
        draw=black}
    }

    \node[state] (vfile) {\doc};
       
    \node[state, rounded corners, right of=vfile, node distance=1.5cm, yshift=1cm] (sertok) {\sertok};
    \node[state, rounded corners, right of=vfile, node distance=1.5cm, yshift=-1cm] (sercomp) {\sercomp};

    \node[state, right of=sertok, node distance=2cm] (toksexp) {Token~\sexps};
    \node[state, right of=sercomp, node distance=2cm] (astsexp) {AST~\sexps};

    \node[state, rounded corners, right of=toksexp, node distance=2cm] (proc) {\postproc};

    \node[state, below of=proc, node distance=1cm] (proctok) {Proc~tokens};

    \node[state, rounded corners, right of=astsexp, node distance=2cm] (learn) {learner};

    \node[state, right of=learn, right of=learn, node distance=0.8cm] (model1) {model~1};
    \node[state, right of=learn, right of=learn, node distance=0.8cm, yshift=1cm] (model2) {model~2};
    
    \draw[->, >=stealth', auto, thick] (vfile) edge (sertok);
    \draw[->, >=stealth', auto, thick] (vfile) edge (sercomp);

    \draw[->, >=stealth', auto, thick] (sertok) edge (toksexp);
    \draw[->, >=stealth', auto, thick] (sercomp) edge (astsexp);

    \draw[->, >=stealth', auto, thick] (toksexp) edge (proc);
    \draw[->, >=stealth', auto, thick] (proc) edge (proctok);

    \draw[->, >=stealth', auto, thick] (proctok) edge (learn);
    \draw[->, >=stealth', auto, thick] (astsexp) edge (learn);

    \draw[->, >=stealth', auto, thick] (learn) edge (model1);
    \draw[->, >=stealth', auto, thick] (learn) edge (model2);
    
  \end{tikzpicture}
  }
  \vspace{-5pt}
  \caption{Implementation architecture and workflow.}
  \vspace{-15pt}
  \label{fig:toolchain}
\end{figure}

